2.4-THz Bandwidth Optical Coherent Receiver Based on a Photonic Crystal Microcomb

We demonstrate a spectrally-sliced single-polarization optical coherent receiver with a record 2.4-THz bandwidth, using a 200-GHz tantalum pentoxide photonic crystal microring resonator as the local oscillator frequency comb.

==> figs/results_fig2.tex <==
\begin{tikzpicture}
\begin{axis} [ylabel=SNR,
              xlabel=Tx number,
              grid=both,
 %             ymin=-60,ymax=10,
 %             xmin=191,xmax=196.4,
              cycle list/Set1,
              ylabel near ticks,
              width = \linewidth,
              ymin = 11,
              ymax = 30,
              legend pos = north east,
              height = 0.5*\linewidth,
             legend style={font=\footnotesize},
                label style={font=\footnotesize},
               tick label style={font=\footnotesize}]
%              yticklabels={0,10,20,30,40,50,60,70,80},
%              ytick={0,10,20,30,40,50,60,70,80}]

\addplot+ [thick] table [x=Tx no, y=SNR recovered, col sep=comma] {data/SNRs_est.csv};
\addlegendentry{Recovered SNR}

\addplot+ [mark=*] table [x=Tx no, y=SNR_total, col sep=comma] {data/SNRs_est.csv};
\addlegendentry{Spectrum SNR estimate}

\addplot+ [mark=*] table [x=Tx no, y=SNR penalty, col sep=comma] {data/SNRs_est.csv};
\addlegendentry{Non-spectrum SNR contribution}

\draw[dashed,black,thick] (2,100) -- (2,-100);
\draw[dashed,black,thick] (4,100) -- (4,-100);
\draw[dashed,black,thick] (6,100) -- (6,-100);
\draw[dashed,black,thick] (8,100) -- (8,-100);
\draw[dashed,black,thick] (10,100) -- (10,-100);
\draw[dashed,black,thick] (12,100) -- (12,-100);
\draw[dashed,black,thick] (14,100) -- (14,-100);
\draw[dashed,black,thick] (16,100) -- (16,-100);
\draw[dashed,black,thick] (18,100) -- (18,-100);
\draw[dashed,black,thick] (20,100) -- (20,-100);
\draw[dashed,black,thick] (22,100) -- (22,-100);



\end{axis}
\end{tikzpicture}
